Budget-Smoothed Analysis for Submodular Maximization

The greedy algorithm for monotone submodular function maximization subject to cardinality constraint is guaranteed to approximate the optimal solution to within a $1-1/e$ factor. Although it is well known that this guarantee is essentially tight in the worst case -- for greedy and in fact any efficient algorithm, experiments show that greedy performs better in practice. We observe that for many applications in practice, the empirical distribution of the budgets (i.e., cardinality constraints) is supported on a wide range, and moreover, all the existing hardness results in theory break under a large perturbation of the budget. To understand the effect of the budget from both algorithmic and hardness perspectives, we introduce a new notion of budget smoothed analysis. We prove that greedy is optimal for every budget distribution, and we give a characterization for the worst-case submodular functions. Based on these results, we show that on the algorithmic side, under realistic budget distributions, greedy and related algorithms enjoy provably better approximation guarantees, that hold even for worst-case functions, and on the hardness side, there exist hard functions that are fairly robust to all the budget distributions.

==> old_intro.tex <==
% !TeX root = main.tex

Monotone submodular function maximization subject to a cardinality constraint is a fundamental problem in combinatorial optimization with a wide variety of applications including feature selection, sensor placement, influence maximization in social networks, document summarization, etc. (see e.g.~\cite{KG14} and references therein). We will use influence maximization in social networks as a running example: an advertiser has a limited budget of $k$ free product samples that she wishes to distribute to seed consumers, who will then propagate the news about the product to their friends, then their friends' friends, etc. 
The standard approach to this problem~\cite{KKT15} models the expected final reach of the campaign as a monotone submodular function $f:\cP([n]) \rightarrow \mathbb{R}$ of the set of seed consumers (where $[n]$ is the set of all users in the network).
The goal of the optimization problem is to find a set of $k$ seed consumers that (approximately) maximizes $f$. 

Classic work shows that the simple greedy algorithm achieves a $1-1/e$-approximaiton to the optimal solution in the worst case~\cite{NemhauserWF78}. Furthermore, this bound is tight for algorithms that make sub-exponential queries to the function~\cite{NemhauserW78,Vondrak13}; 
and even succinctly representable functions (e.g. simple models of influence propagation on a social network graph) do not allow better approximation algorithms unless $\P=\NP$~\cite{Feige98}.
In theory, this tight characterization of the optimal approximation factor is very satisfying.

Given the importance of this problem in practical applications, it is also interesting to ask what is the optimal approximation factor that can be obtained on realistic instances. As one can expect, the performance of the greedy algorithm tends to be significantly better in practice (e.g.~\cite{TSP20}). 
When reasoning about real-world instances, there is a natural tradeoff between quality and generality of the guarantees: at one extreme, worst-case analysis only gives a $(1-1/e)$-approximation but applies to every instance; at the other extreme we could, in principle%
\footnote{In general calculating the approximation factor on a real-world instance requires computing the value of the optimal solution; but if we could do that efficiently, we wouldn't need the greedy algorithm in the first place.}, empirically evaluate the exact performance of the greedy algorithm on each instance of interest, but we would have to redo this for every new instance.
 Our goal in this work is to provide the {\em simplest possible explanation for better-than-$(1-1/e)$-approximation in practice}. I.e.~we want to extend the classic worst-case model --while making minimal assumptions-- to explain why efficient algorithms like greedy should obtain better approximation factors. %If the assumptions underlying such a model are realistic, they could guide us towards designing even better algorithms.

Coming up with useful and realistic assumptions about submodular functions continues to be an interesting and active topic of research. In Section~\ref{sec:related} we survey several natural restrictions, including recent success stories that allow for improved approximation algorithms~\cite{KL14,SviridenkoVW17,BRS16,HorelS16,Yoshida16,CRV17,TSP20,STY20}. Deferring details for later, we argue that the bottom line of this discussion is that submodular functions are complex  objects, and as such modeling their beyond-worst-case behavior is tricky and often application-dependent.

In this work, we circumvent the complexity of modeling typical submodular functions by focusing on the beyond-worst-case behavior of a much simpler object: the cardinality constraint. 
Namely, inspired by the celebrated smoothed analysis~\cite{SpielmanT04}, we
initiate the study of submodular function maximization in a {\em budget-smoothed analysis}. We show that without making any assumptions about the submodular function%
\footnote{Except monotonicity.}
, we can make significant progress by merely perturbing the cardinality constraint.

Clearly, tiny perturbations of the constraint cannot escape the hardness of approximation results%
\footnote{By submodularity, a $(1+\eps)$-multiplicative perturbation in budget cannot affect the value of the solution by more than a $(1+\eps)$-factor.}. Instead we consider larger perturbations, e.g.~budget drawn uniformly from $[x,10x]$ for some $x$. 
To motivate this assumption, consider a small and a large social marketing campaigns. While they both advertise and propagate on the same social network (hence maximize essentially the same, possibly worst-case, submodular function), their budgets can easily differ by an order of magnitude or more. Thus even if the social network/submodular function is worst case, the ``average'' advertiser uses an ``average'' budget which is independent of the social network/submodular function.


\subsection*{The budget-smoothed analysis model}
We study monotone submodular function maximization subject to a cardinality constraint in the following semi-adversarial setting:
\begin{definition}[Budget smoothed analysis] \hfill

\begin{enumerate}
\item The distribution $\tilde{\cD}$ of budgets (e.g. uniform over $[x,10x]$) is given as input to the adversary.
\item The adversary chooses a (monotone submodular) function $f$.
\item The cardinality constraint $k \sim \tilde{\cD}$ is drawn at random and given as input to the algorithm.
\item The algorithm (approximately) maximizes $f$ over all sets of size at most $k$.
\end{enumerate}
For any distribution $\tilde{\cD}$, we're interested in the expected ratio $\cR_{ALG}(f,\tilde{\cD})$ between the value obtained by the algorithm and the optimal solution,
$$ \cR_{ALG}(f,\tilde{\cD}):=\E_{k \sim \tilde{\cD}}\left[\frac{f(ALG)}{f(OPT)}\right].$$
\label{def:budget_smoothed}
\end{definition}


We focus on algorithms that do not assume knowledge of $\tilde{\cD}$, but, somewhat surprisingly, they will be competitive with algorithms that know $\tilde{\cD}$.

Naturally the approximation factors we obtain will depend on the distribution $\tilde{\cD}$. For example, as we explained above, if $\tilde{\cD}$ is concentrated in a small multiplicative interval $[x,(1+\eps)x]$, we cannot hope to get more than a $(1+\eps)$-factor advantage.

For notational convenience, we make the following change to the above model: Rather than sampling the budget from a distribution, each instance will be characterized by a base budget $k_0$ and a {\em budget perturbation distribution} $\cD$, with the final cardinality constraint being $k:= \rho \cdot k_0$ for $\rho \sim \cD$. This will allow us to talk about a distribution $\cD$ like ``uniform over $[x,10x]$'' while studying the asymptotic complexity as the instance size and cardinality constraint go to infinity.


\subsection*{Our results}
In our model of budget-smoothed analysis, we investigate the following questions: Is it possible to obtain better approximation factors? If so, how much better compared to the worst-case $1-1/e$? Are simple algorithms like Greedy still optimal?


\begin{remark*}
All the hardness results below hold both in the black-box oracle model (for any algorithm that makes a subexponential number of queries), or assuming $\P\neq\NP$ in the computational model for coverage functions (on a polynomial-size graph).
\end{remark*} 


\paragraph{Result 1: Optimal approximation factors}
For any budget perturbation distribution $\cD$, we characterize the optimal possible approximation factor as a simple (but non-convex) optimization program  (Section~\ref{sec:simulation}). We also include some numerical estimates for natural distributions (Table~\ref{table:simulation_result}).
In particular, we see that {\em our analysis guarantees non-negligible improvements even for worst-case submodular functions.}
For the special case of $\cD$ supported on two budgets, we also give a closed-form solution (Proposition~\ref{prop:two_budget}). 



\paragraph{Result 2: Optimal approximation algorithms}
We prove that a large class of algorithms that are (near-)optimal in the worst-case continue to obtain (near-)optimal approximation factors under budget-smoothed analysis for {\em any} distribution (Observation~\ref{obs:opt_algorithms} and Appendix~\ref{sec:practical_algorithms}). This class includes the simple greedy algorithms, as well as (variants of) recent efficient parallel algorithms, and Map-Reduce algorithms. In particular, these algorithms are optimal even in comparison to algorithms that know the budget perturbation distribution $\cD$. % This class includes the simple greedy algorithms, as well as (variants of) recent nearly-linear time algorithms, efficient parallel algorithms, and streaming algorithms. In particular, these algorithms are optimal even in comparison to algorithms that know the budget distribution $\cD$.



\paragraph{Result 3: Bounding the best-case budget distribution}
We also prove that for every budget distribution and any efficient algorithm, the optimal budget-smoothed analysis approximation factor is bounded away from $1$ (in particular, it is at most $0.9087$). %\footnote{We were quite surprised to discover that the optimal approximation factor is bounded away from $1$.}.


\begin{table}%[h!]
\begin{center}
\caption{\label{table:simulation_result} Empirical Results}
\begin{tabular}{ |c|c| } 
 \hline
{\bf  Budget perturbation distribution} & \textbf{Worst-case approximation ratio} \\

 \hline
 Baseline (no perturbation) &  0.6321\\
 \hline
  \hline
 Uniform over $[1,10]$ & 0.6675 \\
 Log-scale-uniform over $[1,10]$ & 0.6674 \\ 
 Log-scale-uniform over $[1,600]$ & 0.6808 \\ 
% uniform & 0.66998 \\
 \hline
% Gaussian & 0.66055 \\
Top 10 social/political campaigns on Facebook & 0.6625 \\
 2020 Democratic presidential candidates & 0.6727 \\
 \hline
\end{tabular}
\end{center}
We calculated tight approximation factors for worst-case monotone submodular functions for several exemplary budget distributions. See Section~\ref{sub:numerical} for details. 
% \Aviad{TBD: Update}The 1st distribution is Uniform\{$1.1^{-i}\mid i=0,\dots,24$\}, and the 2nd is Uniform\{$(3i+8)/80\mid i=0,\dots,24$\}. The 3rd distribution is Uniform\{$1.4^{-i}\mid i=0,\dots,19$\}, and the 4th is Uniform\{$(599i/19+1)/600\mid i=0,\dots,19$\}. The 5th is uniform over $25$ budgets sampled from Gaussian distribution $\mathcal{N}(\frac{1}{2},\frac{1}{36})$. The 6th distribution is uniform over the total spent of democrat candidates in 2020 US presidential election from Oct. 1 to Dec. 31, 2019~\cite{2020election}. The last distribution is uniform over the top ten amount spent during the month before Mar. 26, 2020 in the Facebook Ad report~\cite{2020facebook}.
\end{table} 


\subsection{Discussion and future directions}
At a super high level, our results show that while the worst-case approximation factor for monotone submodular maximization is $\approx 0.63$, our new model can explain, under minimal assumptions, why we should expect at least $\approx 0.67$.
\begin{quote}
Is improving submodular maximization approximation from $0.63$ to $0.67$ significant?
\end{quote}
First, we believe that given the vast interest in this problem, this improvement already interesting. 
Clearly, it is insufficient to fully explain the success of greedy on real world instances; 
without making any assumptions on the submodular function, it would be very ambitious to expect that%
\footnote{Although we did expect the approximation factor to be higher given that our budget perturbations completely shatter known hardness construction. We find the robustness of our new hardness constructions quite surprising.} in a first attempt.  
For comparison,~\cite{SpielmanT04}'s original polynomial upper bound for smoothed analysis (of a non-trivial variant) of the Simplex algorithm was $\tilde{O}(d^{55}n^{86}\sigma^{-30} + d^{70}n^{86})$%
\footnote{Here $d$ is the number of variables, $n$ is the number of constraints, and $\sigma^2$ is the variance of the perturbation, see~\cite{DH18}.} iterations...
Indeed, we believe that there are countless future directions to explore in our new model of budget-smoothed analysis.
To exhibit this breadth of possibilities, we mention a couple of preliminary results that we have for other problems that fit into our new model:
\begin{itemize}
\item Submodular maximization subject to {\em knapsack constraint}. While the optimal $1-1/e$ factor can again be recovered in polynomial time, the state-of-the-art algorithms for this problem are still not completely satisfying~\cite{Sviridenko04,EN19,NS20}, and the greedy algorithm does not provide any non-trivial approximation guarantee. Our preliminary results show that with budget-smoothed analysis, greedy guarantees a constant factor approximation with knapsack constraint, and in fact to date we haven't been able to rule out $1-1/e$ approximation (or better).
\item Budget-feasible mechanism design: this is a well-studied problem in AGT~\cite{singer2010budget,chen2011approximability,DobzinskiPS11,BadanidiyuruKS12,SingerM13,ChanC14,EG14,GoelNS14,HorelIM14,BalkanskiH16,ChanC16,NushiS0K16,ZhaoLM16,ZhengWGZTC17,LeonardiMSZ17,anari2018budget,KhalilabadiT18,AmanatidisKS19,gravin2019optimal,LiZY20}. Under a large market assumption~\cite{anari2018budget} obtain a mechanism with optimal approximation guarantee, incidentally also $1-1/e$. Our preliminary results show that this mechanism does {\em not} improve at all under budget-smoothed analysis, but this inspires a {\em new mechanism} that is optimal under budget-smoothed analysis and also significantly outperforms~\cite{anari2018budget}'s mechanism on realistic distributions theoretically and empirically. 
\end{itemize} 

\subsection{Roadmap}
In Section~\ref{sec:related} we survey several other approaches to beyond-worst-case submodular functions. In Section~\ref{sec:greedy} we prove our core technical result% (which is also quite simple)
, namely that greedy obtains optimal approximation factors for any distribution; in Appendix~\ref{sec:practical_algorithms} we extend this result to other related algorithms. In the following sections we build on these techniques; in particular we henceforth simply analyze the approximation factors of the greedy algorithm. In Section~\ref{sec:bound}, we prove %the second part of Result 1, namely 
that the optimal approximation factor is bounded away from $1$ for any distribution. In Section~\ref{sec:simulation}, we %obtain Result 2, namely the 
characterize the optimal approximation factor. We then use this program to simulate several exemplary distributions. %Finally, in Appendix~\ref{sec:2-budgets} we give an explicit formula for the optimal approximation factor with two budgets.%, including the lower bound example mentioned in Result 1.


\subsection{Beyond-worst-case submodular functions}\label{sec:related}
Due to the popularity of submodular maximization in practice, there is a lot of interest in understanding and designing algorithms for ``typical'' cases.
We discuss a few approaches below. 
We note that our model of beyond-worst-case {\em constraint} is orthogonal to any assumptions about the submodular function, and in principle could be combined with any of them to obtain even stronger results.

The model most closely in spirit to our smoothed-analysis-like approach is to take a worst-case submodular function and perturb it with random noise. 
The most straightforward way of doing this is independently perturbing the value of the function for each set. Unfortunately, this breaks the submodularity, which makes the problem significantly {\em harder}, even for small perturbations:~\cite{HS17}barely recover the $1-1/e$ approximation factor in this setting (under further restrictions and with a technically involved algorithm).

Another approach is to consider {\em coverage functions}, an important special class of monotone submodular functions. This restriction has been successful for learning submodular functions~\cite{BalcanCIW12, BadanidiyuruDFKNR12, FeldmanK14}, but Feige's \NP-hard instance already rules out efficient algorithms with improved approximation ratios for this case.
One may combine this restriction with perturbations of the weights of the elements of the ground set; but it is not hard to show that Feige's instance can be made robust even to very large amounts of noise.
Another alternative is to consider special classes of graphs, e.g. power law, small-world, or triangle-dense that are common for social networks ~\cite{WS98,GRS16}. But again Feige's instance either already satisfies all of those, or can be adapted to do so.

Another popular restriction of monotone submodular functions is {\em bounded curvature}~\cite{CC84}, which restricts the extent to which ground elements interact; this indeed allows for better algorithms with applications to e.g.~maximum entropy sampling~\cite{CC84,SviridenkoVW17,BRS16,HorelS16,Yoshida16}. But bounded curvature seems too restrictive for applications like influence in social networks and consumers' valuations with diminishing returns%
\footnote{If, for example, we already selected all of a node's neighbors, the  marginal contribution of adding this node is diminished to zero. For consumers' valuations, the marginal contribution of, e.g. the one-thousandth apple, is again diminished to essentially zero. This means that curvature is unbounded in both settings (see~\cite{CC84,SviridenkoVW17} for formal definitions).}.

To cope with the limited applicability of curvature, the original paper of \cite{CC84} also defined a relaxed notion of {\em greedy curvature}, which only restricts the interaction between elements selected by the greedy algorithm and elements in the optimal solution. In exciting recent work,~\cite{TSP20} define various notions of {\em sharpness} which only restricts the interactions of the average element of the optimal solution. Both greedy curvature and sharpness parameters suffer from the disadvantage that they may be intractable to compute (both are assumptions about interaction of elements with the optimal solutions, and if we knew the optimal soluion...). Moreover, due to their complicated form it's hard to heuristically reason about their fit for any particular application. Nevertheless, on the positive side both are more realistic than vanilla curvature assumption, and combining them with our budget-smoothed analysis model is an interesting direction for future research.

\cite{CRV17} study submodular maximization under a {\em stability} assumption, i.e.~they assume that the optimal subset does not change when the function is perturbed. 
\cite{TSP20} argue that in the context of submodular maximization, stable instances may fail to capture significant interaction between elements. As in the case of greedy curvature and sharpness, it is also not clear how to compute the stability of a function, or reason about instances that we expect to be stable.

Finally, one setting that is both natural and allows for improved approximation factors is influence maximization in undirected graphs~\cite{KL14, ST19, STY20}. Specifically,~\cite{KL14} prove that the greedy algorithm obtains a $(1-1/e+\varepsilon)$-approximation (for some small unspecified constant $\varepsilon>0$) for the independent cascade model on undirected graph. \cite{STY20} show that in the linear threshold model the greedy algorithm does not beat the $(1-1/e)$-approximation factor (by any constant, in the worst case). 
